Consistent User-Traffic Allocation and Load Balancing in Mobile Edge Caching

Cache-equipped Base-Stations (CBSs) is an attractive alternative to offload the rapidly growing backhaul traffic in a mobile network. New 5G technology and dense femtocell enable one user to connect to multiple base-stations simultaneously. Practical implementation requires the caches in BSs to be regarded as a cache server, but few of the existing works considered how to offload traffic, or how to schedule HTTP requests to CBSs. In this work, we propose a DNS-based HTTP traffic allocation framework. It schedules user traffic among multiple CBSs by DNS resolution, with the consideration of load-balancing, traffic allocation consistency and scheduling granularity of DNS. To address these issues, we formulate the user-traffic allocation problem in DNS-based mobile edge caching, aiming at maximizing QoS gain and allocation consistency while maintaining load balance. Then we present a simple greedy algorithm which gives a more consistent solution when user-traffic changes dynamically. Theoretical analysis proves that it is within 3/4 of the optimal solution. Extensive evaluations in numerical and trace-driven situations show that the greedy algorithm can avoid about 50% unnecessary shift in user-traffic allocation, yield more stable cache hit ratio and balance the load between CBSs without losing much of the QoS gain.

==> sections/p1top2.tex <==
\subsection{Relaxation of Equality Constraints}
%There are equality constraints \eqref{LM:3} in $P1$, implying the inherent need of CDN that every map unit must be assigned to a server, which may lead to the insolubility.
%of $P1$ when the capacity of all the CDN servers is insufficient:

For most of the cases, the total capacity of all the CDN edge servers is sufficient to meet all the demands, which ensures $P1$ has feasible solution(s) and thus the optimal solution(s). As a corollary, Lemma~\ref{lemma1} shows that a necessary condition for $P1$'s solubility is the sufficiency of CDNs' total capacity:

\begin{lemma}
\label{lemma1}
If $P1$ has any feasible solution, $\sum_{j\in\mathbf{M}}c_j\geq\lambda_0\sum_{i\in\mathbf{U}}|\mathbf{K_i}|$.
\end{lemma}

\begin{proof}[Proof]
See Appendix~\ref{prooflemma1}
\end{proof}

$\sum_{j\in\mathbf{M}}c_j$ and $\lambda_0\sum_{i\in\mathbf{U}}|\mathbf{K_i}|$ represents the total capacity and demand, respectively. Lemma~\ref{lemma1} helps us to prove the equivalency between $P1$ and the new model obtained by relaxing the equality constraints \eqref{LM:3}, namely, $P2$. 

\begin{theo}
\label{p1top2}
If $P1$ has any feasible solution, the optimal solutions of $P2$ are exactly the same as those of $P1$, where $P2$ is described as follows:
\begin{subequations}
\label{p2}
\begin{alignat}{2}
\nonumber&{P2}\\
\max\quad & \mu_1 Q(\mathbf{X})+\mu_2 B(\mathbf{X})+\mu_3 D(\mathbf{X}) \label{OM:1}\\
\mbox{s.t.}\quad &L_j(\mathbf{X})\leq c_j, \forall j\in\mathbf{M}\label{OM:2}\\
&\sum_{j\in\mathbf{M}}x^k_{ij}\leq 1, \forall i\in\mathbf{U},k\in\mathbf{K}\label{OM:3}\\
&x_{ij}^k\in\{0,1\}, \forall i\in\mathbf{U},j\in\mathbf{M},k\in\mathbf{K}\label{OM:4}
\end{alignat}
\end{subequations}
\end{theo}

\begin{proof}[Proof]
See Appendix~\ref{proofp1top2}
\end{proof}

Theorem~\ref{p1top2} indicates that $P1$ and $P2$ are equivalent as long as $P1$ has any feasible solution, which is reasonably assumed, and thus we are able to solve $P1$ by solving $P2$.

\subsection{Proof of Lemma \ref{lemma1}}
\label{prooflemma1}
\begin{proof}[Proof]
Let $\mathbf{\tilde{X}}=[\tilde{x}_{ij}^k]$ be a feasible solution of $P1$. Then we have $L_j(\mathbf{\tilde{X}})\leq c_j, \forall j\in\mathbf{M}$, and therefore $\sum_{j\in\mathbf{M}}L_j(\mathbf{\tilde{X}})=\lambda_0\sum_{i\in\mathbf{N}}\sum_{k\in\mathbf{K_i}}\sum_{j\in\mathbf{M}}\tilde{x}^k_{ij}\overset{\eqref{LM:3}}{=}\lambda_0\sum_{i\in\mathbf{N}}|\mathbf{K_i}|\overset{\eqref{LM:2}}{\leq}\sum_{j\in\mathbf{M}}c_j$.
\end{proof}

\subsection{Proof of Theorem \ref{p1top2}}
\label{proofp1top2}
\begin{proof}[Proof]
If $\mathbf{\ddot{X}}=[\ddot{x}_{ij}^k]$ is an optimal solution of $P2$ but not of $P1$, $\mathbf{\ddot{X}}$ must be a solution satisfying \eqref{OM:3} but not \eqref{LM:3}, which means:

\begin{equation}
\exists \langle i_0, k_0\rangle, \sum_{j\in\mathbf{M}}x^{k_0}_{i_0j}=0
\label{co1}
\end{equation}

If $P1$ has any feasible solution, there must be $j_0$ with $L_{j_0}(\mathbf{\ddot{X}})<c_{j_0}$, otherwise $L_j(\mathbf{\ddot{X}})=c_j$ for all $j\in\mathbf{M}$, which contradicts \eqref{co1} as $\lambda_0(\sum_{i\in\mathbf{N}}|\mathbf{K_i}|-1)\overset{\eqref{co1}}{\geq}
\lambda_0(\sum_{i\neq i_0 \vee k\neq k_0}\sum_{j\in\mathbf{M}}\ddot{x}^k_{ij}+\sum_{j\in\mathbf{M}}\ddot{x}^{k_0}_{i_0j})=\sum_{j\in\mathbf{M}}L_j(\mathbf{\ddot{X}})=\sum_{j\in\mathbf{M}}c_j\overset{Lemma~\ref{lemma1}}{\geq}\lambda_0\sum_{i\in\mathbf{N}}|\mathbf{K_i}|$. Let $\ddot{x}^{k_0}_{i_0j_0}$ be from 0 to 1. Constraints $L_{j_0}(\mathbf{\ddot{X}})\leq c_{j_0}$ remains satisfied and \eqref{OM:1} will increase, which contradicts the fact that $\mathbf{\ddot{X}}$ is the optimal solution of $P2$. Therefore, if $P1$ has any feasible solution, all optimal solutions of $P2$ and $P1$ must be the same.
\end{proof}

